A crystalline incarnation of Berthelot's conjecture and K\"unneth formula for isocrystals

Berthelot's conjecture predicts that under a proper and smooth morphism of schemes in characteristic $p$, the higher direct images of an overconvergent $F$-isocrystal are overconvergent $F$-isocrystals. In this paper we prove that this is true for crystals up to isogeny. As an application we prove a K\"unneth formula for the crystalline fundamental group.

==> packages_and_functions.for_preamble.tex <==
\usepackage{extarrow}
\usepackage{enumerate}
\usepackage{fontenc}
\usepackage[T1]{fontenc}
\usepackage{graphicx}
\usepackage[colorlinks=true, linkcolor=blue]{hyperref}
\usepackage{latexsym}
\usepackage{mathrsfs}
\usepackage{mathtext}
\usepackage{tikz}
\usepackage{textcomp}
\usepackage{upgreek}
\usepackage{xy}


\usetikzlibrary{arrows}
\usetikzlibrary{matrix}
\usetikzlibrary{shapes}
\usetikzlibrary{snakes}
\usetikzlibrary{matrix}














\DeclareMathOperator{\Add}{\textup{Add}}
%\DeclareMathOperator{\Aff}{\textup{Aff}}
\DeclareMathOperator{\Alg}{\textup{Alg}}
\DeclareMathOperator{\Ann}{\textup{Ann}}
\DeclareMathOperator{\Arr}{\textup{Arr}}
\DeclareMathOperator{\Art}{\textup{Art}}
\DeclareMathOperator{\Ass}{\textup{Ass}}
%\DeclareMathOperator{\Aut}{\textup{Aut}}
\DeclareMathOperator{\Autsh}{\underline{\textup{Aut}}}
\DeclareMathOperator{\Bi}{\textup{B}}
\DeclareMathOperator{\CAdd}{\textup{CAdd}}
\DeclareMathOperator{\CAlg}{\textup{CAlg}}
\DeclareMathOperator{\CMon}{\textup{CMon}}
\DeclareMathOperator{\CPMon}{\textup{CPMon}}
\DeclareMathOperator{\CRings}{\textup{CRings}}
\DeclareMathOperator{\CSMon}{\textup{CSMon}}
\DeclareMathOperator{\CaCl}{\textup{CaCl}}
\DeclareMathOperator{\Cart}{\textup{Cart}}
\DeclareMathOperator{\Cl}{\textup{Cl}}
\DeclareMathOperator{\Coh}{\textup{Coh}}
\DeclareMathOperator{\Coker}{\textup{Coker}}
%\DeclareMathOperator{\Cov}{\textup{Cov}}
\DeclareMathOperator{\Der}{\textup{Der}}
%\DeclareMathOperator{\Div}{\textup{Div}}
\DeclareMathOperator{\End}{\textup{End}}
\DeclareMathOperator{\Endsh}{\underline{\textup{End}}}
\DeclareMathOperator{\Ext}{\textup{Ext}}
\DeclareMathOperator{\Extsh}{\underline{\textup{Ext}}}
\DeclareMathOperator{\FAdd}{\textup{FAdd}}
\DeclareMathOperator{\FCoh}{\textup{FCoh}}
\DeclareMathOperator{\FGrad}{\textup{FGrad}}
\DeclareMathOperator{\FLoc}{\textup{FLoc}}
\DeclareMathOperator{\FMod}{\textup{FMod}}
\DeclareMathOperator{\FPMon}{\textup{FPMon}}
\DeclareMathOperator{\FRep}{\textup{FRep}}
\DeclareMathOperator{\FSMon}{\textup{FSMon}}
\DeclareMathOperator{\FVect}{\textup{FVect}}
\DeclareMathOperator{\Fibr}{\textup{Fibr}}
\DeclareMathOperator{\Fix}{\textup{Fix}}
\DeclareMathOperator{\Fl}{\textup{Fl}}
\DeclareMathOperator{\Fr}{\textup{Fr}}
\DeclareMathOperator{\Funct}{\textup{Funct}}
\DeclareMathOperator{\GAlg}{\textup{GAlg}}
\DeclareMathOperator{\GExt}{\textup{GExt}}
\DeclareMathOperator{\GHom}{\textup{GHom}}
\DeclareMathOperator{\GL}{\textup{GL}}
\DeclareMathOperator{\GMod}{\textup{GMod}}
\DeclareMathOperator{\GRis}{\textup{GRis}}
\DeclareMathOperator{\GRiv}{\textup{GRiv}}
%\DeclareMathOperator{\Gal}{\textup{Gal}}
\DeclareMathOperator{\Gl}{\textup{Gl}}
\DeclareMathOperator{\Grad}{\textup{Grad}}
\DeclareMathOperator{\Hilb}{\textup{Hilb}}
\DeclareMathOperator{\Hl}{\textup{H}}
%\DeclareMathOperator{\Hom}{\textup{Hom}}
\DeclareMathOperator{\Homsh}{\underline{\textup{Hom}}}
\DeclareMathOperator{\ISym}{\textup{Sym}^*}
\DeclareMathOperator{\Imm}{\textup{Im}}
\DeclareMathOperator{\Irr}{\textup{Irr}}
\DeclareMathOperator{\Iso}{\textup{Iso}}
\DeclareMathOperator{\Isosh}{\underline{\textup{Iso}}}
%\DeclareMathOperator{\Ker}{\textup{Ker}}
\DeclareMathOperator{\LAdd}{\textup{LAdd}}
\DeclareMathOperator{\LAlg}{\textup{LAlg}}
\DeclareMathOperator{\LMon}{\textup{LMon}}
\DeclareMathOperator{\LPMon}{\textup{LPMon}}
\DeclareMathOperator{\LRings}{\textup{LRings}}
\DeclareMathOperator{\LSMon}{\textup{LSMon}}
\DeclareMathOperator{\Left}{\textup{L}}
\DeclareMathOperator{\Lex}{\textup{Lex}}
%\DeclareMathOperator{\Loc}{\textup{Loc}}
%\DeclareMathOperator{\M}{\textup{M}}
\DeclareMathOperator{\ML}{\textup{ML}}
\DeclareMathOperator{\MLex}{\textup{MLex}}
%\DeclareMathOperator{\Map}{\textup{Map}}
%\DeclareMathOperator{\Mod}{\textup{Mod}}
\DeclareMathOperator{\Mon}{\textup{Mon}}
\DeclareMathOperator{\Ob}{\textup{Ob}}
\DeclareMathOperator{\Obj}{\textup{Obj}}
\DeclareMathOperator{\PDiv}{\textup{PDiv}}
\DeclareMathOperator{\PGL}{\textup{PGL}}
\DeclareMathOperator{\PML}{\textup{PML}}
\DeclareMathOperator{\PMLex}{\textup{PMLex}}
\DeclareMathOperator{\PMon}{\textup{PMon}}
%\DeclareMathOperator{\Pic}{\textup{Pic}}
\DeclareMathOperator{\Picsh}{\underline{\textup{Pic}}}
\DeclareMathOperator{\Pro}{\textup{Pro}}
\DeclareMathOperator{\Proj}{\textup{Proj}}
\DeclareMathOperator{\QAdd}{\textup{QAdd}}
\DeclareMathOperator{\QAlg}{\textup{QAlg}}
\DeclareMathOperator{\QCoh}{\textup{QCoh}}
\DeclareMathOperator{\QMon}{\textup{QMon}}
\DeclareMathOperator{\QPMon}{\textup{QPMon}}
\DeclareMathOperator{\QRings}{\textup{QRings}}
\DeclareMathOperator{\QSMon}{\textup{QSMon}}
%\DeclareMathOperator{\R}{\textup{R}}
%\DeclareMathOperator{\Rep}{\textup{Rep}}
\DeclareMathOperator{\Rings}{\textup{Rings}}
\DeclareMathOperator{\Riv}{\textup{Riv}}
\DeclareMathOperator{\SFibr}{\textup{SFibr}}
\DeclareMathOperator{\SMLex}{\textup{SMLex}}
\DeclareMathOperator{\SMex}{\textup{SMex}}
\DeclareMathOperator{\SMon}{\textup{SMon}}
\DeclareMathOperator{\SchI}{\textup{SchI}}
\DeclareMathOperator{\Sh}{\textup{Sh}}
\DeclareMathOperator{\Soc}{\textup{Soc}}
%\DeclareMathOperator{\Spec}{\textup{Spec}}
\DeclareMathOperator{\Specsh}{\underline{\textup{Spec}}}
\DeclareMathOperator{\Stab}{\textup{Stab}}
\DeclareMathOperator{\Supp}{\textup{Supp}}
\DeclareMathOperator{\Sym}{\textup{Sym}}
\DeclareMathOperator{\TMod}{\textup{TMod}}
\DeclareMathOperator{\Top}{\textup{Top}}
\DeclareMathOperator{\Tor}{\textup{Tor}}
%\DeclareMathOperator{\Vect}{\textup{Vect}}
\DeclareMathOperator{\alt}{\textup{ht}}
\DeclareMathOperator{\car}{\textup{char}}
%\DeclareMathOperator{\codim}{\textup{codim}}
\DeclareMathOperator{\degtr}{\textup{degtr}}
\DeclareMathOperator{\depth}{\textup{depth}}
\DeclareMathOperator{\divis}{\textup{div}}
\DeclareMathOperator{\et}{\textup{et}}
\DeclareMathOperator{\ffpSch}{\textup{ffpSch}}
\DeclareMathOperator{\h}{\textup{h}}
\DeclareMathOperator{\ilim}{\displaystyle{\lim_{\longrightarrow}}}
%\DeclareMathOperator{\ind}{\textup{ind}}
\DeclareMathOperator{\indim}{\textup{inj dim}}
\DeclareMathOperator{\lf}{\textup{LF}}
\DeclareMathOperator{\op}{\textup{op}}
\DeclareMathOperator{\ord}{\textup{ord}}
\DeclareMathOperator{\pd}{\textup{pd}}
\DeclareMathOperator{\plim}{\displaystyle{\lim_{\longleftarrow}}}
\DeclareMathOperator{\pr}{\textup{pr}}
\DeclareMathOperator{\pt}{\textup{pt}}
\DeclareMathOperator{\rk}{\textup{rk}}
\DeclareMathOperator{\tr}{\textup{tr}}
\DeclareMathOperator{\type}{\textup{r}}
\DeclareMathOperator*{\colim}{\textup{colim}}

==> packages_and_functions.tex <==
\global\long\def\A{\mathbb{A}}


\global\long\def\Ab{(\textup{Ab})}


\global\long\def\C{\mathbb{C}}


\global\long\def\Cat{(\textup{cat})}


\global\long\def\Di#1{\textup{D}(#1)}


\global\long\def\E{\mathcal{E}}


\global\long\def\F{\mathbb{F}}


\global\long\def\GCov{G\textup{-Cov}}


\global\long\def\Gcat{(\textup{Galois cat})}


\global\long\def\Gfsets#1{#1\textup{-fsets}}


\global\long\def\Gm{\mathbb{G}_{m}}


\global\long\def\GrCov#1{\textup{D}(#1)\textup{-Cov}}


\global\long\def\Grp{(\textup{Grps})}


\global\long\def\Gsets#1{(#1\textup{-sets})}


\global\long\def\HCov{H\textup{-Cov}}


\global\long\def\MCov{\textup{D}(M)\textup{-Cov}}


\global\long\def\MHilb{M\textup{-Hilb}}


\global\long\def\N{\mathbb{N}}


\global\long\def\PGor{\textup{PGor}}


\global\long\def\PGrp{(\textup{Profinite Grp})}


\global\long\def\PP{\mathbb{P}}


\global\long\def\Pj{\mathbb{P}}


\global\long\def\Q{\mathbb{Q}}


\global\long\def\RCov#1{#1\textup{-Cov}}


\global\long\def\RR{\mathbb{R}}


\global\long\def\Sch{\textup{Sch}}


\global\long\def\WW{\textup{W}}


\global\long\def\Z{\mathbb{Z}}


\global\long\def\acts{\curvearrowright}


\global\long\def\alA{\mathscr{A}}


\global\long\def\alB{\mathscr{B}}


\global\long\def\arr{\longrightarrow}


\global\long\def\arrdi#1{\xlongrightarrow{#1}}


\global\long\def\catC{\mathscr{C}}


\global\long\def\catD{\mathscr{D}}


\global\long\def\catF{\mathscr{F}}


\global\long\def\catG{\mathscr{G}}


\global\long\def\comma{,\ }


\global\long\def\covU{\mathcal{U}}


\global\long\def\covV{\mathcal{V}}


\global\long\def\covW{\mathcal{W}}


\global\long\def\duale#1{{#1}^{\vee}}


\global\long\def\fasc#1{\widetilde{#1}}


\global\long\def\fsets{(\textup{f-sets})}


\global\long\def\iL{r\mathscr{L}}


\global\long\def\id{\textup{id}}


\global\long\def\la{\langle}


\global\long\def\odi#1{\mathcal{O}_{#1}}


\global\long\def\ra{\rangle}


\global\long\def\set{(\textup{Sets})}


\global\long\def\sets{(\textup{Sets})}


\global\long\def\shA{\mathcal{A}}


\global\long\def\shB{\mathcal{B}}


\global\long\def\shC{\mathcal{C}}


\global\long\def\shD{\mathcal{D}}


\global\long\def\shE{\mathcal{E}}


\global\long\def\shF{\mathcal{F}}


\global\long\def\shG{\mathcal{G}}


\global\long\def\shH{\mathcal{H}}


\global\long\def\shI{\mathcal{I}}


\global\long\def\shJ{\mathcal{J}}


\global\long\def\shK{\mathcal{K}}


\global\long\def\shL{\mathcal{L}}


\global\long\def\shM{\mathcal{M}}


\global\long\def\shN{\mathcal{N}}


\global\long\def\shO{\mathcal{O}}


\global\long\def\shP{\mathcal{P}}


\global\long\def\shQ{\mathcal{Q}}


\global\long\def\shR{\mathcal{R}}


\global\long\def\shS{\mathcal{S}}


\global\long\def\shT{\mathcal{T}}


\global\long\def\shU{\mathcal{U}}


\global\long\def\shV{\mathcal{V}}


\global\long\def\shW{\mathcal{W}}


\global\long\def\shX{\mathcal{X}}


\global\long\def\shY{\mathcal{Y}}


\global\long\def\shZ{\mathcal{Z}}


\global\long\def\st{\ | \ }


\global\long\def\stA{\mathcal{A}}


\global\long\def\stB{\mathcal{B}}


\global\long\def\stC{\mathcal{C}}


\global\long\def\stD{\mathcal{D}}


\global\long\def\stE{\mathcal{E}}


\global\long\def\stF{\mathcal{F}}


\global\long\def\stG{\mathcal{G}}


\global\long\def\stH{\mathcal{H}}


\global\long\def\stI{\mathcal{I}}


\global\long\def\stJ{\mathcal{J}}


\global\long\def\stK{\mathcal{K}}


\global\long\def\stL{\mathcal{L}}


\global\long\def\stM{\mathcal{M}}


\global\long\def\stN{\mathcal{N}}


\global\long\def\stO{\mathcal{O}}


\global\long\def\stP{\mathcal{P}}


\global\long\def\stQ{\mathcal{Q}}


\global\long\def\stR{\mathcal{R}}


\global\long\def\stS{\mathcal{S}}


\global\long\def\stT{\mathcal{T}}


\global\long\def\stU{\mathcal{U}}


\global\long\def\stV{\mathcal{V}}


\global\long\def\stW{\mathcal{W}}


\global\long\def\stX{\mathcal{X}}


\global\long\def\stY{\mathcal{Y}}


\global\long\def\stZ{\mathcal{Z}}


\global\long\def\then{\ \Longrightarrow\ }


\global\long\def\L{\textup{L}}


\global\long\def\l{\textup{l}}



